Impact of Transceiver Impairments on the Capacity of Dual-Hop Relay Massive MIMO Systems

Despite the deleterious effect of hardware impairments on communication systems, most prior works have not investigated their impact on widely used relay systems. Most importantly, the application of inexpensive transceivers, being prone to hardware impairments, is the most cost-efficient way for the implementation of massive multiple-input multiple-output (MIMO) systems. Consequently, the direction of this paper is towards the investigation of the impact of hardware impairments on MIMO relay networks with large number of antennas. Specifically, we obtain the general expression for the ergodic capacity of dual-hop (DH) amplify-and-forward (AF) relay systems. Next, given the advantages of the free probability (FP) theory with comparison to other known techniques in the area of large random matrix theory, we pursue a large limit analysis in terms of number of antennas and users by shedding light to the behavior of relay systems inflicted by hardware impairments.

==> def.tex <==
\usepackage{calc}




% \usepackage[normalem]{ulem}
% \usepackage{url}
% \usepackage{hyperref}
% \hypersetup{colorlinks,urlcolor=blue}

% \hypersetup{colorlinks=false,pdfborder=000}

\makeatletter
% \DeclareUrlCommand\ULurl@@{%
%   \def\UrlFont{\ttfamily\color{blue}}%
%   \def\UrlLeft{\uline\bgroup}%
%   \def\UrlRight{\egroup}}
% \def\ULurl@#1{\hyper@linkurl{\ULurl@@{#1}}{#1}}
% \DeclareRobustCommand*\ULurl{\hyper@normalise\ULurl@}

%\pagenumbering{arabic}
% Package includes
\usepackage{xcolor,multirow,gensymb}
  \usepackage{cite}
\usepackage{graphicx,subfigure,epsfig}
\usepackage{psfrag}
\usepackage{amsmath,amssymb}
\usepackage{color}
\usepackage{array}
\usepackage{nicefrac}
\interdisplaylinepenalty=2500
%\include{preamble_global}
%++++++++++++++++++++++++++++++

\usepackage{amsmath,amssymb}
\usepackage{xifthen}
\usepackage{mathtools}
\usepackage{enumerate}
\usepackage{microtype}
\usepackage{xspace}
%\usepackage[noadjust]{cite}
\usepackage{bm}
\usepackage[T1]{fontenc}
%\usepackage[francais]{babel}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{rotating}
\usepackage{tabulary}
\usepackage{float}

\newfloat{longequation}{b}{ext}

\newfloat{eq.}{t}{ext}

% \usepackage{cleveref}

% vectors and matrices
\newcommand{\vect}[1]{{\lowercase{\mbs{#1}}}}
\renewcommand{\deg}{\degree}


%definition of identity matrix I have to redefine \bm below in mathbb(m)
\newcommand{\mbs}[1]{\bm{#1}}
\newcommand{\mat}[1]{{\uppercase{\mbs{#1}}}}
\newcommand{\Id}{\mat{\mathrm{I}}}


\renewcommand{\Bmatrix}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\Pmatrix}[1]{\begin{pmatrix}#1\end{pmatrix}}

% transpose, Hermitian  transpose
\newcommand{\T}{{\scriptscriptstyle\mathsf{T}}}
\renewcommand{\H}{{\scriptscriptstyle\mathsf{H}}}
%\newcommand{\h}{{\scriptscriptstyle\mathsf{H}}}

\newcommand{\cond}{\,\vert\,}
\renewcommand{\Re}[1][]{\ifthenelse{\isempty{#1}}{\operatorname{Re}}{\operatorname{Re}\left(#1\right)}}
\renewcommand{\Im}[1][]{\ifthenelse{\isempty{#1}}{\operatorname{Im}}{\operatorname{Im}\left(#1\right)}}


\newcommand{\av}{\vect{a}}
\newcommand{\bv}{\vect{b}}
\newcommand{\cv}{\vect{c}}
\newcommand{\dv}{\vect{d}}
\newcommand{\ev}{\vect{e}}
\newcommand{\fv}{\vect{f}}
\newcommand{\gv}{\vect{g}}
\newcommand{\hv}{\vect{h}}
\newcommand{\iv}{\vect{i}}
\newcommand{\jv}{\vect{j}}
\newcommand{\kv}{\vect{k}}
\newcommand{\lv}{\vect{l}}
\newcommand{\mv}{\vect{m}}
\newcommand{\nv}{\vect{n}}
\newcommand{\ov}{\vect{o}}
\newcommand{\pv}{\vect{p}}
\newcommand{\qv}{\vect{q}}
\newcommand{\rv}{\vect{r}}
\newcommand{\sv}{\vect{s}}
\newcommand{\tv}{\vect{t}}
\newcommand{\uv}{\vect{u}}
\newcommand{\vv}{\vect{v}}
\newcommand{\wv}{\vect{w}}
\newcommand{\xv}{\vect{x}}
\newcommand{\yv}{\vect{y}}
\newcommand{\zv}{\vect{z}}
\newcommand{\zerov}{\vect{0}}
\newcommand{\etv}{\vect{\eta}}
\def\var{{\mathrm{var}}}


\newcommand{\nuv}{\vect{\nu}}
\newcommand{\deltav}{\hbox{\boldmath$\delta$}}
\newcommand{\Phim}{\pmb{\Phi}}
\newcommand{\Psim}{\pmb{\Psi}}

\newcommand{\Am}{\mat{a}}
\newcommand{\Bm}{\mat{b}}
\newcommand{\Cm}{\mat{c}}
\newcommand{\Dm}{\mat{d}}
\newcommand{\Em}{\mat{e}}
\newcommand{\Fm}{\mat{f}}
\newcommand{\Gm}{\mat{g}}
\newcommand{\Hm}{\mat{h}}
\newcommand{\Idd}{{\bf I}}
%\renewcommand{\Im}{\mat{i}}
\newcommand{\Jm}{\mat{j}}
\newcommand{\Km}{\mat{k}}
\newcommand{\Lm}{\mat{l}}
\newcommand{\Mm}{\mat{M}}
\newcommand{\Nm}{\mat{n}}
\newcommand{\Om}{\mat{o}}
\newcommand{\Pm}{\mat{p}}
\newcommand{\Qm}{\mat{q}}
\newcommand{\Rm}{\mat{r}}
\newcommand{\Sm}{\mat{s}}
\newcommand{\Um}{\mat{u}}
\newcommand{\Vm}{\mat{V}}
\newcommand{\Wm}{\mat{w}}
\newcommand{\Xm}{\mat{x}}
\newcommand{\ym}{\mat{y}}

% Bold capital letters
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}
\def\bSigma{{\mathbf{\Sigma}}}


% Caligraphic capital letters
\def\cA{{\mathcal{A}}}
\def\cB{{\mathcal{B}}}
\newcommand{\cC}{{\cal C}}
\def\cD{{\mathcal{D}}}
\def\cE{{\mathcal{E}}}
\def\cF{{\mathcal{F}}}
\def\cG{{\mathcal{G}}}
\def\cH{{\mathcal{H}}}
\def\cI{{\mathcal{I}}}
\def\cJ{{\mathcal{J}}}
\def\cK{{\mathcal{K}}}
\def\cL{{\mathcal{L}}}
\def\cM{{\mathcal{M}}}
\newcommand{\cN}{{\cal N}}
\def\cO{{\mathcal{O}}}
\def\cP{{\mathcal{P}}}
\def\cQ{{\mathcal{Q}}}
\def\cR{{\mathcal{R}}}
\def\cS{{\mathcal{S}}}
\def\cT{{\mathcal{T}}}
\def\cU{{\mathcal{U}}}
\def\cV{{\mathcal{V}}}
\def\cW{{\mathcal{W}}}
\def\cX{{\mathcal{X}}}
\def\cY{{\mathcal{Y}}}
\def\cZ{{\mathcal{Z}}}
\def\cd{{\mathcal{d}}}

% Caligraphic lowercase letters
\def\ra{{\mathrm{a}}}
\def\rb{{\mathrm{b}}}
\def\rc{{\mathrm{c}}}
\def\rd{{\mathrm{d}}}
\def\re{{\mathrm{e}}}
\def\rf{{\mathrm{f}}}
\def\rg{{\mathrm{g}}}
\def\rh{{\mathrm{h}}}
\def\ri{{\mathrm{i}}}
\def\rj{{\mathrm{j}}}
\def\rk{{\mathrm{k}}}
\def\rl{{\mathrm{l}}}
\def\rn{{\mathrm{n}}}
\def\ro{{\mathrm{o}}}
\def\rp{{\mathrm{p}}}
\def\rq{{\mathrm{q}}}
\def\rr{{\mathrm{r}}}
\def\rs{{\mathrm{s}}}
\def\rt{{\mathrm{t}}}
\def\ru{{\mathrm{u}}}
\def\rv{{\mathrm{v}}}
\def\rw{{\mathrm{w}}}
\def\rx{{\mathrm{x}}}
\def\ry{{\mathrm{y}}}
\def\rz{{\mathrm{z}}}


% Bold lowercase
\def\bydef{:=}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\bee{{\mathbf{e}}}
\def\bff{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bi{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bmm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}
\def\b0{{\mathbf{0}}}
\def\bONE{{\mathbf{1}}}
\def\bTheta{{\boldsymbol{\Theta}}}

\newcommand{\htp}{^{\sf H}}
\newcommand{\Zm}{{\bf Z}}
\newcommand{\Tm}{{\bf T}}
\newcommand{\barvH}{\bar{\bH}}
\def\bbC{{\mathbb{C}}}
\def\rr{{\mathrm{r}}}
\newcommand{\Nc}{{\cal N}}
\def\bpsi{{\boldsymbol{\psi}}}
\def\bPsi{{\boldsymbol{\Psi}}}



\newcommand{\CC}{\mathbb{C}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\EE}{\mathbb{E}}

\newcommand{\one}{\mat{\mathrm{1}}}

\newcommand{\CN}[1][]{\ifthenelse{\isempty{#1}}{\mathcal{N}_{\mathbb{C}}}{\mathcal{N}_{\mathbb{C}}\left(#1\right)}}
\def\rf{{\mathrm{f}}}

\renewcommand{\P}[1][]{\ifthenelse{\isempty{#1}}{\mathbb{P}}{\mathbb{P}\left(#1\right)}}
\newcommand{\E}[1][]{\ifthenelse{\isempty{#1}}{\mathbb{E}}{\mathbb{E}\left(#1\right)}}
\renewcommand{\det}[1][]{\ifthenelse{\isempty{#1}}{\text{det}}{\text{det}\left(#1\right)}}
\newcommand{\trace}[1][]{\ifthenelse{\isempty{#1}}{\text{tr}}{\text{tr}\left(#1\right)}}
\newcommand{\rank}[1][]{\ifthenelse{\isempty{#1}}{\text{rank}}{\text{rank}\left(#1\right)}}
\newcommand{\diag}[1][]{\ifthenelse{\isempty{#1}}{\text{diag}}{\text{diag}\left(#1\right)}}
\def\nn{\nonumber}


\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\normf{\lVert}{\rVert_{\text{F}}}
\IEEEoverridecommandlockouts

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem, Definition, ...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\defeq}{\triangleq}
\newcommand{\eqdef}{\triangleq}

\newtheorem{proposition}{Proposition}%[section]
\newtheorem{remark}{Remark}%ti[section]
\newtheorem{definition}{Definition}%[section]
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{example}{Example}%[section]
\newtheorem{corollary}{Corollary}%[section]
\newtheorem{conjecture}{Conjecture}%[section]
\newtheorem{fact}{Fact}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{assumption}{Assumption}%[section]
\newcommand{\barvR}{\bar{\bR}}
\newcommand{\hatvH}{\hat{\bH}} 
\newcommand{\hatvh}{\hat{\bh}} 
\newcommand{\barvh}{\bar{\bh}}
\newcommand{\hatvg}{\hat{\bg}} 
\newcommand{\hatvG}{\hat{\bG}} 
\def\bPhi{{\boldsymbol{\Phi}}}
\def\bPsi{{\boldsymbol{\Psi}}}

\newcommand{\brevevh}{\breve{\bh}}  
\newcommand{\tr}{\mathop{\mathrm{tr}}\nolimits}
\newtheorem{Theorem}{Theorem}

\newcommand{\al}{\alpha}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Answer & Solution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{enumi_saved}
\setcounter{enumi_saved}{0}

\newenvironment{question}
{
\begin{enumerate}[Q1.]
    \setcounter{enumi}{\value{enumi_saved}}
}
{
\setcounter{enumi_saved}{\value{enumi}}
\end{enumerate}
}


\usepackage{answers}
\Newassociation{solution}{Solution}{solutionfile}
\renewcommand{\solutionextension}{sln}
\renewcommand{\Solutionparams}{{ Q\Currentlabel.}}
\renewcommand{\solutionstyle}[1]{#1}
\AtBeginDocument{\Opensolutionfile{solutionfile}[\jobname]}
\AtEndDocument{\Closesolutionfile{solutionfile}\clearpage
%\section*{Solutions}%
%\pagestyle{empty}\input{\jobname.sln}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Really Optional
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
